Polyglot Code Smell Detection for Infrastructure as Code with GLITCH

This paper presents GLITCH, a new technology-agnostic framework that enables automated polyglot code smell detection for Infrastructure as Code scripts. GLITCH uses an intermediate representation on which different code smell detectors can be defined. It currently supports the detection of nine security smells and nine design & implementation smells in scripts written in Ansible, Chef, Docker, Puppet, or Terraform. Studies conducted with GLITCH not only show that GLITCH can reduce the effort of writing code smell analyses for multiple IaC technologies, but also that it has higher precision and recall than current state-of-the-art tools. A video describing and demonstrating GLITCH is available at: https://youtu.be/E4RhCcZjWbk

==> arxiv/_abstract.tex <==
%Infrastructure as Code (IaC) is a process that facilitates the provision of scalable and reproducible environments. Due to its wide use and importance, there have been several efforts to automatically detect code smells in IaC scripts. However, and even though many code smells are technology-agnostic, most efforts tend to focus on a specific IaC technology. This means that when the detection of a new smell is implemented in one of the tools, it is not immediately available for the technologies supported by the other tools\,---\,the only option is to duplicate the effort.
%To address this challenge, we present \GLITCH, a new technology-agnostic framework that enables automated polyglot smell detection by transforming IaC scripts into an intermediate representation, on which different smell detectors can be defined. \GLITCH\ currently supports the detection of \numsecsmells\ different security smells and \numdesimpsmells\ design \& implementation smells in scripts written in Puppet, Ansible, or Chef.
This paper presents \GLITCH, a new technology-agnostic framework that enables automated polyglot code smell detection for Infrastructure as Code scripts. \GLITCH\ uses an intermediate representation on which different code smell detectors can be defined. It currently supports the detection of \numsecsmells\ security smells and \numdesimpsmells\ design \& implementation smells in scripts written in Ansible, Chef, Docker, Puppet, or Terraform.
%We compare \GLITCH\ with state-of-the-art smell detectors. The results obtained 
Studies conducted with \GLITCH\ not only show that \GLITCH\ can reduce the effort of writing code smell analyses for multiple IaC technologies, but also that it has higher precision and recall than current state-of-the-art tools. 
A video describing and demonstrating \GLITCH\ is available at: \url{https://youtu.be/E4RhCcZjWbk}.
